WELES: Policy-driven Runtime Integrity Enforcement of Virtual Machines

Trust is of paramount concern for tenants to deploy their security-sensitive services in the cloud. The integrity of VMs in which these services are deployed needs to be ensured even in the presence of powerful adversaries with administrative access to the cloud. Traditional approaches for solving this challenge leverage trusted computing techniques, e.g., vTPM, or hardware CPU extensions, e.g., AMD SEV. But, they are vulnerable to powerful adversaries, or they provide only load time (not runtime) integrity measurements of VMs. We propose WELES, a protocol allowing tenants to establish and maintain trust in VM runtime integrity of software and its configuration. WELES is transparent to the VM configuration and setup. It performs an implicit attestation of VMs during a secure login and binds the VM integrity state with the secure connection. Our prototype's evaluation shows that WELES is practical and incurs low performance overhead.

==> tables/load_times.tex <==
\begin{table}[t!]
\caption{
    Read times of files depending on their size. When a file is open for the first time, it is measured by IMA and the measurement digest is extended to the emulated TPM. 
}
\vspace{\captiontablevspacesize}
\center
\begin{tabular}{lllll}
File size & \specialcell{VM \\ 1st read} & \specialcell{VM \\ next read} & \specialcell{Host \\ 1st read} & \specialcell{Host \\ next read} \\ \hline
10 B & 48 ms ($\sigma=6$) & 21 $\mu$s (sd=4) & 12 ms (sd=0) & 21 $\mu$s (sd=4) \\
100 B & 63 ms (sd=11) & 22 $\mu$s (sd=1) & 11 ms (sd=0) & 20 $\mu$s (sd=1) \\
1 KiB & 66 ms (sd=12) & 22 $\mu$s (sd=1) & 12 ms (sd=1) & 20 $\mu$s (sd=1) \\
10 KiB & 69 ms (sd=13) & 22 $\mu$s (sd=1) & 12 ms (sd=0) & 20 $\mu$s (sd=0) \\
100 KiB & 68 ms (sd=10) & 23 $\mu$s (sd=1) & 13 ms (sd=0) & 20 $\mu$s (sd=1) \\
1 MiB & 87 ms (sd=7) & 22 $\mu$s (sd=1) & 45 ms (sd=102) & 20 $\mu$s (sd=0) \\
10 MiB & 134 ms (sd=2) & 23 $\mu$s (sd=1) & 179 ms (sd=184) & 20 $\mu$s (sd=0)  \\
100 MiB & 630 ms (sd=5) & 23 $\mu$s (sd=1) & 570 ms (sd=164) & 20 $\mu$s (sd=1)  \\
1 GiB & 5548 ms (sd=19) & 23 $\mu$s (sd=1) & 4131 ms (sd=180) & 20 $\mu$s (sd=0)  \\
\hline
\end{tabular}
\label{tab:eval:ima_read_latency}
\end{table}


==> tables/mc_max_writes.tex <==
\begin{table}[t!]
\vspace{2mm}
\caption{
  The TPM 2.0 chips does not seem to have problems of TPM 1.2 chips, which have limited number of MC increments.
}
\vspace{\captiontablevspacesize}
\center
\begin{tabular}{lm{3cm}cc}
  \textbf{} & Counter value & Slowdown \\ \hline
discrete TPM & 85M & no slowdown \\
integrated TPM & 8M & after 7.3M \\
\end{tabular}
\label{tab:eval:mc_max_writes}
\end{table}

